Tight Lower Bounds on Worst-Case Guarantees for Zero-Shot Learning with Attributes

We develop a rigorous mathematical analysis of zero-shot learning with attributes. In this setting, the goal is to label novel classes with no training data, only detectors for attributes and a description of how those attributes are correlated with the target classes, called the class-attribute matrix. We develop the first non-trivial lower bound on the worst-case error of the best map from attributes to classes for this setting, even with perfect attribute detectors. The lower bound characterizes the theoretical intrinsic difficulty of the zero-shot problem based on the available information -- the class-attribute matrix -- and the bound is practically computable from it. Our lower bound is tight, as we show that we can always find a randomized map from attributes to classes whose expected error is upper bounded by the value of the lower bound. We show that our analysis can be predictive of how standard zero-shot methods behave in practice, including which classes will likely be confused with others.

==> tables/all.tex <==
\begin{table*}[ht]
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{lcccccccccccccccccccc}
    \toprule
    Method &  \multicolumn{4}{c}{AwA2} & \multicolumn{4}{c}{aPY} & \multicolumn{4}{c}{CUB} & \multicolumn{4}{c}{SUN} & \multicolumn{4}{c}{LAD}\\
    \midrule
    & Top-1 & U & S & H & Top-1 & U & S & H & Top-1 & U & S & H & Top-1 & U & S & H & Top-1 & U & S & H\\
    \cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13} \cmidrule(lr){14-17} \cmidrule(lr){18-21}
    DAP & 65.22 & 49.45 & 85.51 & 62.67 & 28.30 & 8.72 & 54.28 & 15.02 & 22.27 & 4.94 & 14.36 & 7.35 & 19.65 & 5.28 & 5.92 & 5.58 & - & - & - & - \\
    ESZSL & 54.82 & 4.04 & 88.83 & 7.72 & 38.56 &  2.25 & 81.07 & 4.39 & 53.95 & 14.71 & 56.53 & 23.33 & 55.69 & 13.75 & 28.41 & 18.53& 25.25 & 8.07 & 70.91 & 14.49\\
    SAE & 58.89 & 12.86 & 87.20 & 22.41 & 16.49 & 13.99 & 84.69 & 24.01 & 46.71 & 15.72 & 57.02 & 24.64 & 59.86 & 19.03 & 31.20 & 23.64 & - & - & - & -\\
    DeVISE & 60.25 $\pm$ 2.63 & 8.22 $\pm$ 1.69 & 89.73 $\pm$ 0.66 & 15.02 $\pm$ 2.84 & 33.40 $\pm$ 2.13 & 11.39 $\pm$ 2.19 & 72.58 $\pm$ 1.85 & 19.60 $\pm$ 3.40 & 46.80 $\pm$ 0.94 & 24.20 $\pm$ 0.94 & 61.55 $\pm$ 1.58 & 34.74 $\pm$ 1.22 & 54.74 $\pm$ 1.08 & 19.33 $\pm$ 0.47 & 33.64 $\pm$ 0.76 & 24.54 $\pm$ 0.37 & - & - & - & -\\
    ALE & 52.78 $\pm$ 2.78 & 11.21 $\pm$ 0.24 & 81.18 $\pm$ 0.53 & 19.70 $\pm$ 0.36 & 33.52 $\pm$ 0.35 & 4.01 $\pm$ 1.53 & 76.68 $\pm$ 4.08 & 7.56 $\pm$ 2.71 & 51.38 $\pm$ 0.77 & 26.80 $\pm$ 0.59 & 60.11 $\pm$ 1.89 & 37.05 $\pm$ 0.38 & 61.69 $\pm$ 0.40 & 23.87 $\pm$ 0.72 & 36.13 $\pm$ 0.66 & 28.74 $\pm$ 0.52 & - & - & - & -\\
    SJE & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & -\\
    \midrule
    Adversarial & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & -\\
    \bottomrule
    \end{tabular}}
    \caption{ZSL and GZSL accuracy (\%). For we report the Top-1 balanced average class-accuracy for standard ZSL. For GZSL, we report the average class-accuracy for the unseen (U) and seen (S) classes, together with their harmonic mean (H). All the metrics are obtained on the GBU proposed splits, and the intervals represent the standard errors over 5 seeds. Both ESZSL and SAE do not have intervals because have a closed form solution. SAE shoes results from the semantic to the feature space (reference to section 4.1 of the paper).}
\label{tab:acc:gs_and_fms}
\end{table*}


==> tables/clique_metrics.tex <==
\begin{table}[t]
    \centering
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{lcccccccc}
    \toprule
    Method &  \multicolumn{2}{c}{aPY} & \multicolumn{2}{c}{AwA2} & \multicolumn{2}{c}{CUB} & \multicolumn{2}{c}{SUN}\\
    \midrule
    & \textbf{Prec.} & \textbf{Rec.} & \textbf{Prec}. & \textbf{Rec.}  & \textbf{Prec}. & \textbf{Rec.}  & \textbf{Prec}. & \textbf{Rec.} \\
    \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
    DAP & 1.00 & 0.58 &   0.90 & 0.47  & 0.81 & 0.36  & 0.91 & 0.29  \\
    ESZSL & 1 & 0.62 & 0.82 & 0.47 & 0.84 & 0.35 &  0.97  & 0.27 \\
    SAE & 0.71  & 0.38  & 0.82 & 0.47  & 0.86 & 0.33  &  0.97 & 0.26  \\
    %DeVISE & 0.56  & 0.35 & 4.11 & 0.71  & 0.26 & 2.26  & 0.74 & 0.29 & 3.55 & 0.87 & 0.26 & 3.60 \\
    SJE &  1.00 & 0.61  &  0.88 & 0.37   & 0.81 & 0.35  & 0.97 & 0.27   \\
    ALE & 1.00 &  0.69   & 0.90 & 0.47 & 0.89 & 0.33  & 0.98 & 0.27  \\
    \bottomrule
    \end{tabular}}
    \caption{\Cri{To do}}
\label{tab:metrics_cliques}
\end{table}


==> tables/gzsl.tex <==
\begin{table*}[ht]
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{lcccccccccccccccccccc}
    \toprule
    Method &  \multicolumn{4}{c}{AwA2} & \multicolumn{4}{c}{aPY} & \multicolumn{4}{c}{CUB} & \multicolumn{4}{c}{SUN} & \multicolumn{4}{c}{LAD}\\
    \midrule
    & Top-1 & U & S & H & Top-1 & U & S & H & Top-1 & U & S & H & Top-1 & U & S & H & Top-1 & U & S & H\\
    \cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13} \cmidrule(lr){14-17} \cmidrule(lr){18-21}
    DAP & 65.22 & 49.45 & 85.51 & 62.67 & 28.30 & 8.72 & 54.28 & 15.02 & 22.27 & 4.94 & 14.36 & 7.35 & 19.65 & 5.28 & 5.92 & 5.58 & - & - & - & - \\
    ESZSL & 54.82 & 4.04 & 88.83 & 7.72 & 38.56 &  2.25 & 81.07 & 4.39 & 53.95 & 14.71 & 56.53 & 23.33 & 55.69 & 13.75 & 28.41 & 18.53& 25.25 & 8.07 & 70.91 & 14.49\\
    SAE & 58.89 & 12.86 & 87.20 & 22.41 & 16.49 & 13.99 & 84.69 & 24.01 & 46.71 & 15.72 & 57.02 & 24.64 & 59.86 & 19.03 & 31.20 & 23.64 & - & - & - & -\\
    DeVISE & 60.25 $\pm$ 2.63 & 8.22 $\pm$ 1.69 & 89.73 $\pm$ 0.66 & 15.02 $\pm$ 2.84 & 33.40 $\pm$ 2.13 & 11.39 $\pm$ 2.19 & 72.58 $\pm$ 1.85 & 19.60 $\pm$ 3.40 & 46.80 $\pm$ 0.94 & 24.20 $\pm$ 0.94 & 61.55 $\pm$ 1.58 & 34.74 $\pm$ 1.22 & 54.74 $\pm$ 1.08 & 19.33 $\pm$ 0.47 & 33.64 $\pm$ 0.76 & 24.54 $\pm$ 0.37 & - & - & - & -\\
    ALE & 52.78 $\pm$ 2.78 & 11.21 $\pm$ 0.24 & 81.18 $\pm$ 0.53 & 19.70 $\pm$ 0.36 & 33.52 $\pm$ 0.35 & 4.01 $\pm$ 1.53 & 76.68 $\pm$ 4.08 & 7.56 $\pm$ 2.71 & 51.38 $\pm$ 0.77 & 26.80 $\pm$ 0.59 & 60.11 $\pm$ 1.89 & 37.05 $\pm$ 0.38 & 61.69 $\pm$ 0.40 & 23.87 $\pm$ 0.72 & 36.13 $\pm$ 0.66 & 28.74 $\pm$ 0.52 & - & - & - & -\\
    SJE & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & -\\
    \midrule
    Adversarial & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & -\\
    \bottomrule
    \end{tabular}}
    \caption{ZSL and GZSL accuracy (\%). For we report the Top-1 balanced average class-accuracy for standard ZSL. For GZSL, we report the average class-accuracy for the unseen (U) and seen (S) classes, together with their harmonic mean (H). All the metrics are obtained on the GBU proposed splits, and the intervals represent the standard errors over 5 seeds. Both ESZSL and SAE do not have intervals because have a closed form solution. SAE shoes results from the semantic to the feature space (reference to section 4.1 of the paper).}
\label{tab:acc:gs_and_fms}
\end{table*}

